Private Date Exposure in Facebook and the Impact of Comprehensible Audience Selection Controls

Privacy in Online Social Networks (OSNs) evolved from a niche topic to a broadly discussed issue in a wide variety of media. Nevertheless, OSNs drastically increase the amount of information that can be found about individuals on the web. To estimate the dimension of data leakage in OSNs, we measure the real exposure of user content of 4,182 Facebook users from 102 countries in the most popular OSN, Facebook. We further quantify the impact of a comprehensible privacy control interface that has been shown to extremely decrease configuration efforts as well as misconfiguration in audience selection. Our study highlights the importance of usable security. (i) The total amount of content that is visible to Facebook users does not dramatically decrease by simplifying the audience selection interface, but the composition of the visible content changes. (ii) Which information is uploaded to Facebook as well as which information is shared with whom strongly depends on the user's country of origin.

==> data_description_2_alt.tex <==
\section{Experimental Setup and Dataset Description}
\label{sec:data_description}

In this section, we specify the setup of our study by describing our ethical considerations, the browser extension FPW which has been used to collect the data and the precise data collection methods. To underline the adequacy of our color-coding audience selection interface to be used in this study, we describe essences on the feedback from study participants.  We further depict which and how much data we were able to collect in this study and describe basic user profile statistics of the participants. The bias as a result of a non-random selection of study participants is also discussed in this section.

\subsection{Ethical Considerations}

We protect the privacy of our study participants! Neither the download logfile which we used to estimate the dissemination of the FPW, nor the feedback answers that we collected are linked to individuals. For this study, we asked the FPW users to send us feedback with consent. We explained the reason for collecting the data and allowed users to access and verify the data before sending it to our server. All feedback responses that we used in this study are anonymized. % as much as possible.
We keep the collected data confidential to protect all study participants from deanonymization attempts and do only publish aggregated data. 


\subsection{The Facebook Privacy Watcher}
\label{subsec:fpw}


In Facebook, the user can choose between a number of visibility-levels for each information in her profile, namely: 'Everyone', 'Friends', 'Custom' and 'Only me'. The 'Custom' setting allows users to authorize single friends or groups of friends (\eg ``colleagues'' and ``good friends'') to access certain information. %Grouping friends leads to more efficient adjusting of privacy settings  than selecting each user per profile attribute individually. This reflects the communities of acquaintances a user is part of in the real world and helps to decide quickly, which group of contacts shall be granted access to a certain profile entry.
In previous work \cite{paul2012c4ps}, a new type of interface has been presented, which is based on a color coding (Figure \ref{fig:Example}). The used colors are guided by the well-known traffic light colors, adding blue to represent custom settings. Results of changes (initiated by clicking at the respective color box) are shown instantly for \emph{direct success control} of each action. We used the following color scheme:

\begin{compactitem}
% \setlength{\itemsep}{2pt}
\item \emph{Red:} Visible to nobody
\item \emph{Blue:} Visible to selected friends
\item \emph{Yellow:} Visible to all friends
\item \emph{Green:} Visible to everyone
\end{compactitem}
% 
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.45\textwidth]{grafiken/new_privacy_settings_buttons.png}
% \caption{Example for an attribute's privacy setting (``Birthday: 22. Nov. 1978)}
% \label{fig:Example}
% \end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.36\textwidth]{grafiken/Screenshot8.png}
\caption{Screenshots of photo albums, colorized by the FPW}
\label{fig:screenshot}
\end{figure}

This color scheme is in-line with the sympathy of the majority of the users (Section \ref{subsec:opinions}). Figure \ref{fig:screenshot} shows a screenshot of colorized photo albums as an example for colorized profile fields. Clicking at the colorized boxes changes the privacy settings. A tooltip helps the users to remember the meaning of each color. The color scheme can be adopted to individual user needs. To help color-blind FPW users, we included the possibility to use different stripy patterns instead of colors. The FPW has support for English, German, French, Italian and Arabic.


% Furthermore, we conducted a user study to elaborate whether our new or the original privacy setting interface of Facebook is more intuitive. The results of the user study underlined a clear advantage for the new type of interface. The participants solved all tasks quicker and almost without mistakes.

\subsection{Users' Acceptance of the FPW}
\label{subsec:opinions}

It is essential for the success of the study that participants are willing integrate the tool in their normal OSN usage and to use it more than only once. The FPW and the realized user interface hence need to be both: beneficial for the participants and easily usable.
Thus, the first question which we asked our users in the feedback formula was: ``How do you like the idea of colorizing in this plug-in?''. 

The overwhelming majority rated this idea as ``very good'' (65.66\%) or ``good'' (32.2\%). Less than one percent rated the idea to be ``medium'' (0.98\%), ``bad`` (0.46\%) or ''very bad`` (0.7\%). However, the plug-in did not work from 7th of November 2013, 2:30 am, till 8th of November, 3:30 (am, CET), because of Facebook site changes. During this time, we received most of the negative ratings.


% 0:Very good, 1:Good, 2:Bad, 3:Very bad
% \begin{center}
% \begin{tabular}{lll}
% & Var1 & Freq\\ 
% 1 & 0 & 66.86\\ 
% 2 & 1 & 31.8\\ 
% 3 & 2 & 0.58\\ 
% 4 & 3 & 0.76\\ 
% \end{tabular}
% \end{center}


% \subsection{Color Scheme}

Creating the color scheme, we argued in the team which type of color scheme is more intuitive to the users: green, inspired by traffic lights meaning ``go'' - corresponding in the color scheme to be visible to everybody or green in the meaning of being safe since the item is not visible to anybody. This question has been asked in the previous user study with 40 participants. 60\% of the participants preferred the green to represent the setting meaning 'visible to everybody'. It meets almost perfectly the results in this study (54.83\% vs. 45.17\%).
% 
% Which color scheme is more intuitive?
% 0:Green=Visible for all, 1:Visible only for me
% \begin{center}
% \begin{tabular}{lll}
% & Var1 & Freq\\ 
% 1 & 0 & 58.67\\ 
% 2 & 1 & 41.33\\ 
% \end{tabular}
% \end{center}

% \subsection{Implementation}

The implementation was not rated that good like the idea of using colors for setting privacy. Evaluating the comments, we can find the following reasons: The people who preferred green to represent the safe setting where nobody has access were not satisfied that it was not possible to customize the colors in the first three versions. Furthermore, we suffered from a bug in the first version.

\begin{table}
\small
\centering
\begin{tabular}{rl} \hline
Rating & Percentage\\ \hline
Very good & 32.34\\ 
Good & 61.34\\ 
Medium & 3.44\\
Bad & 1.83\\ 
Very bad  & 1.05\\ \hline
\end{tabular}
\caption{How do you like the implementation of the FPW?}
\end{table}



\subsection{Data Collection}

We gathered data about the FPW from two sources. The first is the download log file at our own server, where the plug-in can be downloaded from. The second source of data is the set of feedback responses which have been sent to us. While the first source gives us insights into the spreading process of the plug-in, the second source allows us to draw a picture of the plug-in usage as well as its impact on privacy settings of the users' profiles.


\subsubsection{Download Log}

% \begin{figure}[ht!]
% \includegraphics[width=0.489\textwidth]{grafiken/feedbacks_per_country.pdf}
% \caption{Feedbacks per country; Top eight countries}
% \label{fig:feedbacks_per_country}
% \end{figure}

Analyzing the download logfile enabled us to understand the time and locality dimensions of the FPW dissemination. We discovered strong peaks subsequently to the moments of publication in different venues as well as that a large user basis is originated in Germany and Egypt. We further discovered a couple of sites, offering to download our plug-in \cite{chip,computerbild,netzwelt,freeware,soft_ware}. Thus, we only have an incomplete view on the actual downloads by analyzing our own download log. Some of those alternative download sites publish the number of downloads. Adding the number of downloads from our site to those external download counters, we estimate the total number of download to be higher than 44,800, coming at least from 102 countries. One year after our first FPW publication, 11,000 users are still following every update that we offer.

% Thus, our statistics just includes the downloads from our own site. The download logfile contains information about the User-Agent settings, the IP of the client which downloaded the file, the host name and the timestamp of the download. An external skript added the Country to our data, based on the IP address.


% \begin{center}
% \begin{tabular}{ll}
% Germany & 13694\\
% Egypt & 3609\\
% Saudi Arabia & 413\\
% Austria & 381\\
% Switzerland & 312\\
% United States & 277\\
% United Arab Emirates & 133\\
% United Kingdom & 112\\
% Syrian Arab Republic & 91\\
% Morocco & 79\\
% \end{tabular}
% \end{center}

% \tp{Todo: add a comparison that shows the total number of downloads each country and compares with the number of feedbacks from each country to show the tendency to send feedbacks; Maybe bar chart with two colors (downloads vs feedbacks)}



\subsubsection{User Feedback}
\label{sec:data_feedbacks}



The usual life-cycle of an FPW instance starts with the installation process and resumes with a check of the privacy settings of the own  profile during a few sessions (1-5). The plug-in is sparely used afterwards. We asked our users to provide us feedback after activating the plug-in three times, which usually happened within the first days after installation. 

We asked for feedback about both: the general idea of coloring the profile items to simplify the privacy settings and the implementation of our plug-in. Furthermore, we offered two text fields to enter comments and suggestions concerning the idea as well as the implementation. 
% Until version 0.69.17 beta, we asked the users to submit the coloring database and the log file of the plug-in for two reasons: some feedbacks contained bug descriptions which could not be solved without detailed information from the log file and the coloring information is a valuable database to investigate the impact of our plug-in.
% 
% Since we received a lot of bug notifications without log file and database, we decided in to make sending the database and log file obligatory for sending feedback. 
We explicitly informed our users about the exact (anonymized) data that we collected. From 2012-10-15 till 2014-07-07,  we received 9,296 feedback responses from 102 countries that included coloring and log file information.

\begin{table}
\small
\centering
\begin{tabular}{rl} \hline
Country & \# Feedback responses \\ \hline
Germany & 7,581 \\ 
Egypt & 272 \\ 
Austria & 218 \\ 
United States & 150 \\
Switzerland & 147 \\ 
France  & 94 \\ 
Spain& 72\\ 
Netherlands & 62\\ 

\hline
\label{tab:numberoffeedbackspercountry}
\end{tabular}
\caption{The number of Feedback responses that we received from the top eight countries}
\end{table}

We collected the following information from our users:

\begin{itemize}
 \item a hash value of the Facebook - UIN
 \item the counter (including timestamps), indicating how often the plug-in was activated
 \item the visibility of each profile field before the first usage of our plug-in happened %(in levels 0-5)
 \item the visibility of each profile field after using our plug-in %(in levels 0-5)
 \item the type and visibility of timeline entries
 \item the number of friends
 \item the number of photos and labels
 \item the number of likes
\end{itemize}



Furthermore, our server, which gathered the feedback data, ran a script to extract the countries from which we received the feedback. %The intention behind storing the profile size metrics (numbers of friends, photos and likes) was to get an idea about who uses our plug-in.



\subsection{Sample Bias and Basic User Profile Statistics}
\label{subsec:sample_bias}

We recruited our sample (FPW users) via an announcement on our homepage and by sending press releases to specialized press. We then witnessed a viral spreading process based on word-of-mouth advertising. The attention of mass media such as news papers \cite{handelsblatt}, radio stations\footnote{\url{http://www.ffh.de/news-service/magazin/toController/Topic/toAction/show/toId/3371/toTopic/die-facebook-ampel-fuer-sichere-postings.html}} and an Egyptian web portal \cite{masrawy} followed afterwards. In spite of the broad audience of the respective media, the set of participants is by no means random. %We also cannot provide 
We decided not to collect detailed demographic informations about FPW users, since this would be inappropriate for a tool that has been advertised to support user's privacy. 
% to collect data on user demographics supports privacy. 
Instead, we provide technical information such as statistics about the user profiles to allow the sample bias to be appraised:


\begin{table}[ht]
\small
\centering
\begin{tabular}{rllll}
  \hline 
 $X$ & $X = 0$ & $ \diameter_{X}$ & $\tilde X$ & $\sigma_{X}$ \\
%   $X$ & $X = 0$ & $\diameter_{X}$ & $\tilde X$ & $\sigma_{X}$ \\ 
  \hline
Friends & 0\% & 148.75 & 96 & 159.53 \\ 
Photos & 3.43\% & 181.69 & 32 & 572.62 \\ 
Labels on Photos & 34.45\% & 20.54 & 3 & 64.45 \\ 
Photo Albums & 3.49\% & 10.71 & 7 & 20.05 \\ 
Locations & 17.07\% & 38.68 & 4 & 101.65 \\ 
Likes & 10.06\% & 90.04 & 36 & 145.33 \\ 
Notes & 86.94\% & 1.49 & 0 & 19.5 \\ 
   \hline
\end{tabular}
\caption{Basic profile statistics: percentage of profiles without any entry in field X and the average, median and standard deviation of the number of entries in field X} 
\label{tab:profile_size}
\end{table}


Our median user has 96 friends, liked 36 pages and shared 32 pictures. Many users have just a few friends (Figure \ref{fig:stats_number_of_friends}) and a few of them have plenty of friends. The degree distribution of the friendship graph as well as the median number of friends is similar to those of the whole Facebook graph \cite{facebook_graph}. We interpret this as an evidence that our FPW users are close to normal with respect to the number of friends. %\tp{ToDo: Compare those numbers with the official numbers from Facebook}


\begin{figure}[ht]
\centering
\includegraphics[width=0.4\textwidth]{grafiken/number_of_friends.png}
\caption{Histogram: number of friends}
\label{fig:stats_number_of_friends}
\end{figure}

% The FPW users from different coutries strongly differ in the number of their friends. We provide the medians and the averages for the eight countries with the most FPW users in Table \ref{tab:friends_country}.
% 
% \begin{table}[h]
% \small
% \centering
% \begin{tabular}{rll} \hline
% Country    &    Mean 	& 	Median 	\\ \hline
% Austria    &	275.83 	&    	193 	\\
% Switzerland &	225.50 	&   	131 	\\
% Germany    & 	154.54  &  	 93 	\\
% Egypt      & 	331.86  &	150 	\\
% Spain      & 	148.78  &	117 	\\
% France     & 	267.81  & 	112 	\\
% Netherlands &	111.63  &   	 90 	\\
% United States & 201.41  & 	115 	\\ \hline
% \end{tabular}
% \caption{Number of friends with respect to countries}
% \label{tab:friends_country}
% \end{table}



% auskommentiert, weil später ohne Varianz. Die Varianz ist redundant, weil die Standardabweichung schon enthalten ist.
% \begin{table}[ht]
% \centering
% \begin{tabular}{rlllll}
%   \hline
% $X$ & $X = 0$ & $\diameter_{X}$ & $\tilde X$ & $Var(X)$ & $\sigma_{X}$ \\ 
%   \hline
% Friends & 0\% & 148.75 & 96 & 25449.93 & 159.53 \\ 
% Photos & 3.43\% & 181.69 & 32 & 327894.4 & 572.62 \\ 
% Labels on Photos & 34.45\% & 20.54 & 3 & 4154.09 & 64.45 \\ 
% Photo Albums & 3.49\% & 10.71 & 7 & 401.9 & 20.05 \\ 
% Locations & 17.07\% & 38.68 & 4 & 10331.83 & 101.65 \\ 
% Likes & 10.06\% & 90.04 & 36 & 21119.63 & 145.33 \\ 
% Notes & 86.94\% & 1.49 & 0 & 380.2 & 19.5 \\ 
%    \hline
% \end{tabular}
% \caption{Basic profile Statistics: percentage of profiles without X, average, median, variance and standard deviation} 
% \label{tab:profile_size}
% \end{table}





% 
% 
% \begin{figure*}[ht!]
% \centering
% \includegraphics[width=0.89\textwidth]{grafiken/stats_number_of_photos.pdf}
% \caption{stats number of photos}
% \label{fig:stats_number_of_photos}
% \end{figure*}

% \begin{figure}[ht!]
% \centering
% \includegraphics[width=0.489\textwidth]{grafiken/timeline_entries_by_type.pdf}
% \caption{timeline\_entries\_by\_type}
% \label{fig:timeline_entries_by_type}
% \end{figure}

